Dynamical traceback age of the $\beta$ Pictoris moving group

Context: The $\beta$ Pictoris moving group is one of the most well-known young associations in the solar neighbourhood and several members are known to host circumstellar discs, planets, and comets. Measuring its age with precision is basic to study several astrophysical processes such as planet formation and disc evolution which are strongly age dependent. Aims: We aim to determine a precise and accurate dynamical traceback age for the $\beta$ Pictoris moving group. Methods: Our sample combines the extremely precise Gaia DR2 astrometry with ground-based radial velocities measured in an homogeneous manner. We use an updated version of our algorithm to determine dynamical ages. The new approach takes into account a robust estimate of the spatial and kinematic covariance matrices of the association to improve the sample selection process and to perform the traceback analysis. Results: We estimate a dynamical age of $18.5_{-2.4}^{+2.0}$ Myr for the $\beta$ Pictoris moving group. We investigated the spatial substructure of the association at birth time and we propose the existence of a core of stars more concentrated. We also provide precise radial velocity measurements for 81 members of $\beta$ Pic, including ten stars with the first determination of their radial velocities. Conclusions: Our dynamical traceback age is three times more precise than previous traceback age estimates and, more important, for the first time, reconciles the traceback age with the most recent estimates of other dynamical, lithium depletion boundary, and isochronal ages. This has been possible thanks to the excellent astrometric and spectroscopic precisions, the homogeneity of our sample, and the detailed analysis of binaries and membership.

==> Tables/19_discarded.tex <==
\begin{table*}[]
    \centering
    \caption{Sources rejected for the study of the $\beta$~Pic dynamical age analysis (see Sect.~\ref{subsec:vel_dist}). All the comments should be taken as possible reasons for which our method discarded the sources.}
    \label{tab:redected}
    \begin{tabular}{c|c|c|l}
    \hline
    \hline
       2MASS ID  &  nSpec & instrument & Comments \\
    \hline
01365516-0647379 &  1 &  FEROS & Poor fit/bin. \\ %
01373545-0645375 &  1 &  HARPS & Contaminant. \\
02232663+2244069 &  1 &  FEROS & Contaminant. \\
03573393+2445106 &  3 & SOPHIE & Binary. \\
05004928+1527006 &  3 & SOPHIE & Contaminant. \\
08475676-7854532 &  1 &   UVES & Contaminant. \\
11493184-7851011 &  2 & FEROS+UVES & Contaminant. \\
13545390-7121476 &  1 &  FEROS & Contaminant. \\
16120516-4556242 &  1 &  FEROS & Contaminant. \\
16181789-2836502 & 36 &  HARPS & Fast rotator. \\ %
17092947-5235197 &  1 &  FEROS & Contaminant. \\
18430597-4058047 &  1 &  FEROS & Contaminant. \\
19312434-2134226 &  1 &  FEROS & Binary. \\
20105054-3844326 &  1 &  FEROS & Contaminant. \\
21212873-6655063 &  1 &  FEROS & Contaminant. \\
23314492-0244395 &  1 &  FEROS & Contaminant. \\
23512227+2344207 &  1 &  FEROS & Binary. \\
21183375+3014346 &  7 & SOPHIE+CAFE & Contaminant. \\
22571130+3639451 &  8 & SOPHIE+CAFE & Spectroscopic binary. \\
    \hline
    \hline
    \end{tabular}
\end{table*}{}

==> Tables/26_members.tex <==
\begin{sidewaystable*}
    \centering
    \caption{Final bona fide sample of 26 members of $\beta$~Pic selected to determine the dynamical age. }
    \label{tab:26_members}

\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|c|}
\hline
\hline
  \multicolumn{1}{|c|}{2MASS ID} &
  \multicolumn{1}{c|}{SpT\tablefootmark{a} (ref)} &
  \multicolumn{1}{c|}{T$_\textup{eff, GDR2}$ (K)} &
  \multicolumn{1}{c|}{$G$ (mag)} &
  \multicolumn{1}{c|}{$X$ (pc)} &
  \multicolumn{1}{c|}{$Y$ (pc)} &
  \multicolumn{1}{c|}{$Z$ (pc)} &
  \multicolumn{1}{c|}{$U$ (km~s$^{-1}$)} &
  \multicolumn{1}{c|}{$V$ (km~s$^{-1}$)} &
  \multicolumn{1}{c|}{$W$ (km~s$^{-1}$)} &
  \multicolumn{1}{c|}{Core}\\
\hline
J00172353-6645124 & M3.0V (1) & 3630 & 11.3 & 14.60 $\pm$ 0.02 & -18.59 $\pm$ 0.02 & -28.21 $\pm$ 0.04 & -10.51 $\pm$ 0.12 & -16.09 $\pm$ 0.15 &  -8.60 $\pm$ 0.22 & Y\\
J04593483+0147007 & M0V   (2) & 3986 &  9.3 &-21.28 $\pm$ 0.02 &  -6.77 $\pm$ 0.01 &  -9.83 $\pm$ 0.01 & -12.42 $\pm$ 0.46 & -16.30 $\pm$ 0.15 &  -9.28 $\pm$ 0.21 & Y\\
J05004714-5715255 & M0V   (2) & 4033 &  9.4 & -1.54 $\pm$ 0.00 & -21.32 $\pm$ 0.02 & -16.33 $\pm$ 0.01 & -11.17 $\pm$ 0.02 & -16.50 $\pm$ 0.15 &  -9.09 $\pm$ 0.12 & Y\\
J05471708-5103594 & A6V   (3) & 7100 &  3.7 & -3.43 $\pm$ 0.02 & -16.65 $\pm$ 0.11 & -10.06 $\pm$ 0.07 & -11.07 $\pm$ 0.96 & -15.79 $\pm$ 4.63 &  -9.21 $\pm$ 2.80 & Y\\
J06182824-7202416 & K4V   (2) & 4555 &  9.3 &  7.59 $\pm$ 0.01 & -33.75 $\pm$ 0.03 & -18.58 $\pm$ 0.02 & -10.50 $\pm$ 0.14 & -16.46 $\pm$ 0.61 &  -8.71 $\pm$ 0.33 & Y\\
J16572029-5343316 & M3    (4) & 3612 & 11.3 & 45.37 $\pm$ 0.28 & -21.65 $\pm$ 0.13 &  -5.88 $\pm$ 0.04 &  -7.35 $\pm$ 0.16 & -15.87 $\pm$ 0.13 & -10.49 $\pm$ 0.08 & N\\
J17020937-6734447 & (M4)  (5) & 3712 & 12.8 & 32.00 $\pm$ 0.05 & -23.67 $\pm$ 0.04 & -10.97 $\pm$ 0.02 &  -8.20 $\pm$ 0.72 & -16.62 $\pm$ 0.53 &  -9.09 $\pm$ 0.25 & N\\
J17024014-4521587 & (M2)  (5) & 3914 & 10.7 & 30.33 $\pm$ 0.06 & -10.06 $\pm$ 0.02 &  -1.24 $\pm$ 0.00 &  -8.67 $\pm$ 0.17 & -16.51 $\pm$ 0.07 & -10.21 $\pm$ 0.03 & Y\\
J17444256-5315471 & (M3)  (5) & 3866 & 12.9 & 48.62 $\pm$ 0.17 & -18.83 $\pm$ 0.07 & -11.34 $\pm$ 0.04 &  -7.17 $\pm$ 0.35 & -16.93 $\pm$ 0.15 & -10.12 $\pm$ 0.09 & N\\
J17483374-5306118 & (M2)  (5) & 3962 & 12.9 & 70.36 $\pm$ 0.29 & -26.64 $\pm$ 0.11 & -16.96 $\pm$ 0.07 &  -7.44 $\pm$ 0.12 & -16.81 $\pm$ 0.09 &  -9.20 $\pm$ 0.06 & Y\\
J18041617-3018280 & (M2)  (5) & 3814 & 11.7 & 54.93 $\pm$ 0.15 &   0.82 $\pm$ 0.00 & - 4.03 $\pm$ 0.01 &  -7.83 $\pm$ 0.24 & -14.52 $\pm$ 0.05 &  -8.45 $\pm$ 0.04 & Y\\
J18055491-5704307 & (M2)  (5) & 3884 & 12.4 & 49.55 $\pm$ 0.16 & -21.31 $\pm$ 0.07 & -16.18 $\pm$ 0.05 &  -8.58 $\pm$ 0.19 & -15.54 $\pm$ 0.10 &  -8.09 $\pm$ 0.07 & Y\\
J18092970-5430532 & (M4)  (5) & 3826 & 13.4 & 34.91 $\pm$ 0.11 & -13.14 $\pm$ 0.04 & -10.76 $\pm$ 0.03 & -10.23 $\pm$ 0.24 & -15.13 $\pm$ 0.11 &  -8.05 $\pm$ 0.08 & N\\
J18161236-5844055 & (M3)  (5) & 3563 & 11.5 & 26.21 $\pm$ 0.05 & -11.84 $\pm$ 0.02 &  -9.68 $\pm$ 0.02 &  -7.78 $\pm$ 0.35 & -17.09 $\pm$ 0.16 & -10.26 $\pm$ 0.13 & N\\
J18281651-4421477 & (M2)  (5) & 3996 & 12.6 & 77.46 $\pm$ 0.28 & -13.26 $\pm$ 0.05 & -20.69 $\pm$ 0.07 &  -6.84 $\pm$ 0.22 & -16.37 $\pm$ 0.08 &  -8.99 $\pm$ 0.08 & Y\\
J18283524-4457280 & (K7)  (5) & 4190 & 11.6 & 79.32 $\pm$ 0.20 & -14.36 $\pm$ 0.04 & -21.66 $\pm$ 0.06 &  -6.45 $\pm$ 0.33 & -16.22 $\pm$ 0.08 &  -8.95 $\pm$ 0.10 & Y\\
J18420694-5554254 & M3.0V (1) & 3753 & 12.4 & 45.01 $\pm$ 0.12 & -16.58 $\pm$ 0.04 & -18.35 $\pm$ 0.05 &  -8.52 $\pm$ 0.19 & -15.40 $\pm$ 0.08 &  -8.28 $\pm$ 0.08 & Y\\
J19225894-5432170 & F6V   (2) & 6437 &  6.9 & 41.30 $\pm$ 0.11 & -12.80 $\pm$ 0.04 & -21.32 $\pm$ 0.06 &  -8.89 $\pm$ 0.34 & -15.43 $\pm$ 0.11 &  -8.06 $\pm$ 0.18 & Y\\
J19233820-4606316 & M0    (4) & 4050 & 11.2 & 64.02 $\pm$ 0.19 &  -9.10 $\pm$ 0.03 & -29.50 $\pm$ 0.09 &  -6.73 $\pm$ 0.74 & -16.37 $\pm$ 0.12 &  -9.76 $\pm$ 0.35 & N\\
J19243494-3442392 & M4.0V (1) & 4045 & 12.8 & 48.13 $\pm$ 0.22 &   3.22 $\pm$ 0.01 & -18.92 $\pm$ 0.09 &  -9.47 $\pm$ 0.58 & -16.14 $\pm$ 0.09 &  -8.88 $\pm$ 0.24 & N\\
J19481651-2720319 & (M2)  (5) & 3944 & 12.2 & 57.78 $\pm$ 0.22 &  13.52 $\pm$ 0.05 & -26.17 $\pm$ 0.10 &  -7.69 $\pm$ 0.15 & -14.99 $\pm$ 0.06 &  -9.20 $\pm$ 0.08 & Y\\
J20013718-3313139 & M1    (4) & 3938 & 11.5 & 52.34 $\pm$ 0.13 &   7.26 $\pm$ 0.02 & -28.47 $\pm$ 0.07 &  -7.68 $\pm$ 0.16 & -15.78 $\pm$ 0.04 &  -9.13 $\pm$ 0.10 & N\\
J20090521-2613265 & F5V   (6) & 6450 &  7.1 & 42.62 $\pm$ 0.09 &  12.23 $\pm$ 0.03 & -23.41 $\pm$ 0.05 &  -6.96 $\pm$ 1.02 & -14.69 $\pm$ 0.29 & -10.27 $\pm$ 0.56 & N\\
J20333759-2556521 & M4.5V (4) & 3864 & 13.1 & 34.55 $\pm$ 0.17 &  11.39 $\pm$ 0.06 & -23.62 $\pm$ 0.12 &  -8.44 $\pm$ 0.76 & -14.85 $\pm$ 0.26 &  -9.59 $\pm$ 0.52 & Y\\
J21100535-1919573 & M2    (4) & 3770 & 10.8 & 21.87 $\pm$ 0.06 &  12.25 $\pm$ 0.04 & -20.26 $\pm$ 0.06 &  -9.91 $\pm$ 0.28 & -15.17 $\pm$ 0.16 &  -9.78 $\pm$ 0.26 & Y\\
J22424896-7142211 & K7V   (2) & 4065 &  9.8 & 19.57 $\pm$ 0.02 & -18.94 $\pm$ 0.02 & -24.54 $\pm$ 0.02 & -10.25 $\pm$ 0.08 & -15.84 $\pm$ 0.08 &  -7.98 $\pm$ 0.10 & Y\\
\hline
\hline
\end{tabular}
\tablebib{ (1)~\citet{Riedel+2017b}; (2)~\citet{Torres+06}; (3)~\citet{Gray+2006}; (4)~\citet{Riaz+2006}; (5)~\citet{Gagne2018b}; (6)~\citet{Houk1982}}
\tablefoot{
\tablefoottext{a}{Spectral types between parentheses were estimated from the absolute $Gaia~G-$band magnitude.}
}
\end{sidewaystable*}{}




% \begin{tabular}{|r|l|c|r|r|r|r|r|r|r|r|}
% \hline
% \hline
%   \multicolumn{1}{|c|}{SourceID\_1} &
%   \multicolumn{1}{c|}{2MASS ID} &
%   \multicolumn{1}{c|}{SpT} &
%   \multicolumn{1}{c|}{RV (km~s$^{-1}$)} &
%   \multicolumn{1}{c|}{G (mag)} &
%   \multicolumn{1}{c|}{X (pc)} &
%   \multicolumn{1}{c|}{Y (pc)} &
%   \multicolumn{1}{c|}{Z (pc)} &
%   \multicolumn{1}{c|}{U (km~s$^{-1}$)} &
%   \multicolumn{1}{c|}{V (km~s$^{-1}$)} &
%   \multicolumn{1}{c|}{W (km~s$^{-1}$)}\\
% \hline
%     4 & 00172353-6645124 & M3   & 10.55 $\pm$ 0.29 & 11.3 & 14.60 $\pm$ 0.02 & -18.59 $\pm$ 0.02 & -28.21 $\pm$ 0.04 & -10.51 $\pm$ 0.12 & -16.09 $\pm$ 0.15 &  -8.60 $\pm$ 0.22\\
%   60 & 04593483+0147007 & M0   & 19.09 $\pm$ 0.53 &  9.3 &-21.28 $\pm$ 0.02 &  -6.77 $\pm$ 0.01 &  -9.83 $\pm$ 0.01 & -12.42 $\pm$ 0.46 & -16.30 $\pm$ 0.15 &  -9.28 $\pm$ 0.21\\
%   61 & 05004714-5715255 & M0   & 19.24 $\pm$ 0.19 &  9.4 & -1.54 $\pm$ 0.00 & -21.32 $\pm$ 0.02 & -16.33 $\pm$ 0.01 & -11.17 $\pm$ 0.02 & -16.50 $\pm$ 0.15 &  -9.09 $\pm$ 0.12\\
%   82 & 05471708-5103594 &      & 19.92 $\pm$ 5.49 &  3.7 & -3.43 $\pm$ 0.02 & -16.65 $\pm$ 0.11 & -10.06 $\pm$ 0.07 & -11.07 $\pm$ 0.96 & -15.79 $\pm$ 4.63 &  -9.21 $\pm$ 2.80\\
%   87 & 06182824-7202416 & K4   & 16.24 $\pm$ 0.71 &  9.3 &  7.59 $\pm$ 0.01 & -33.75 $\pm$ 0.03 & -18.58 $\pm$ 0.02 & -10.50 $\pm$ 0.14 & -16.46 $\pm$ 0.61 &  -8.71 $\pm$ 0.33\\
%   107 & 16572029-5343316 & M3   &  1.42 $\pm$ 0.16 & 11.3 & 45.37 $\pm$ 0.28 & -21.65 $\pm$ 0.13 &  -5.88 $\pm$ 0.04 &  -7.35 $\pm$ 0.16 & -15.87 $\pm$ 0.13 & -10.49 $\pm$ 0.08\\
%   109 & 17020937-6734447 &      &  5.59 $\pm$ 0.93 & 12.8 & 32.00 $\pm$ 0.05 & -23.67 $\pm$ 0.04 & -10.97 $\pm$ 0.02 &  -8.20 $\pm$ 0.72 & -16.62 $\pm$ 0.53 &  -9.09 $\pm$ 0.25\\
%   111 & 17024014-4521587 &      & -2.63 $\pm$ 0.18 & 10.7 & 30.33 $\pm$ 0.06 & -10.06 $\pm$ 0.02 &  -1.24 $\pm$ 0.00 &  -8.67 $\pm$ 0.17 & -16.51 $\pm$ 0.07 & -10.21 $\pm$ 0.03\\
%   120 & 17444256-5315471 &      &  1.59 $\pm$ 0.38 & 12.9 & 48.62 $\pm$ 0.17 & -18.83 $\pm$ 0.07 & -11.34 $\pm$ 0.04 &  -7.17 $\pm$ 0.35 & -16.93 $\pm$ 0.15 & -10.12 $\pm$ 0.09\\
%   122 & 17483374-5306118 &      &  1.04 $\pm$ 0.13 & 12.9 & 70.36 $\pm$ 0.29 & -26.64 $\pm$ 0.11 & -16.96 $\pm$ 0.07 &  -7.44 $\pm$ 0.12 & -16.81 $\pm$ 0.09 &  -9.20 $\pm$ 0.06\\
%   127 & 18041617-3018280 &      & -7.41 $\pm$ 0.24 & 11.7 & 54.93 $\pm$ 0.15 &   0.82 $\pm$ 0.00 & - 4.03 $\pm$ 0.01 &  -7.83 $\pm$ 0.24 & -14.52 $\pm$ 0.05 &  -8.45 $\pm$ 0.04\\
%   128 & 18055491-5704307 &      &  0.65 $\pm$ 0.21 & 12.4 & 49.55 $\pm$ 0.16 & -21.31 $\pm$ 0.07 & -16.18 $\pm$ 0.05 &  -8.58 $\pm$ 0.19 & -15.54 $\pm$ 0.10 &  -8.09 $\pm$ 0.07\\
%   131 & 18092970-5430532 &      & -1.85 $\pm$ 0.27 & 13.4 & 34.91 $\pm$ 0.11 & -13.14 $\pm$ 0.04 & -10.76 $\pm$ 0.03 & -10.23 $\pm$ 0.24 & -15.13 $\pm$ 0.11 &  -8.05 $\pm$ 0.08\\
%   137 & 18161236-5844055 &      &  3.22 $\pm$ 0.41 & 11.5 & 26.21 $\pm$ 0.05 & -11.84 $\pm$ 0.02 &  -9.68 $\pm$ 0.02 &  -7.78 $\pm$ 0.35 & -17.09 $\pm$ 0.16 & -10.26 $\pm$ 0.13\\
%   142 & 18281651-4421477 &      & -1.56 $\pm$ 0.23 & 12.6 & 77.46 $\pm$ 0.28 & -13.26 $\pm$ 0.05 & -20.69 $\pm$ 0.07 &  -6.84 $\pm$ 0.22 & -16.37 $\pm$ 0.08 &  -8.99 $\pm$ 0.08\\
%   144 & 18283524-4457280 &      & -1.02 $\pm$ 0.34 & 11.6 & 79.32 $\pm$ 0.20 & -14.36 $\pm$ 0.04 & -21.66 $\pm$ 0.06 &  -6.45 $\pm$ 0.33 & -16.22 $\pm$ 0.08 &  -8.95 $\pm$ 0.10\\
%   146 & 18420694-5554254 & M3   &  0.47 $\pm$ 0.21 & 12.4 & 45.01 $\pm$ 0.12 & -16.58 $\pm$ 0.04 & -18.35 $\pm$ 0.05 &  -8.52 $\pm$ 0.19 & -15.40 $\pm$ 0.08 &  -8.28 $\pm$ 0.08\\
%   167 & 19225894-5432170 & F6   &  0.05 $\pm$ 0.39 &  6.9 & 41.30 $\pm$ 0.11 & -12.80 $\pm$ 0.04 & -21.32 $\pm$ 0.06 &  -8.89 $\pm$ 0.34 & -15.43 $\pm$ 0.11 &  -8.06 $\pm$ 0.18\\
%   168 & 19233820-4606316 & M0   &  0.08 $\pm$ 0.83 & 11.2 & 64.02 $\pm$ 0.19 &  -9.10 $\pm$ 0.03 & -29.50 $\pm$ 0.09 &  -6.73 $\pm$ 0.74 & -16.37 $\pm$ 0.12 &  -9.76 $\pm$ 0.35\\
%   169 & 19243494-3442392 & M4   & -6.56 $\pm$ 0.63 & 12.8 & 48.13 $\pm$ 0.22 &   3.22 $\pm$ 0.01 & -18.92 $\pm$ 0.09 &  -9.47 $\pm$ 0.58 & -16.14 $\pm$ 0.09 &  -8.88 $\pm$ 0.24\\
%   178 & 19481651-2720319 &      & -6.26 $\pm$ 0.16 & 12.2 & 57.78 $\pm$ 0.22 &  13.52 $\pm$ 0.05 & -26.17 $\pm$ 0.10 &  -7.69 $\pm$ 0.15 & -14.99 $\pm$ 0.06 &  -9.20 $\pm$ 0.08\\
%   184 & 20013718-3313139 & M1   & -4.27 $\pm$ 0.19 & 11.5 & 52.34 $\pm$ 0.13 &   7.26 $\pm$ 0.02 & -28.47 $\pm$ 0.07 &  -7.68 $\pm$ 0.16 & -15.78 $\pm$ 0.04 &  -9.13 $\pm$ 0.10\\
%   187 & 20090521-2613265 & F5   & -4.71 $\pm$ 1.20 &  7.1 & 42.62 $\pm$ 0.09 &  12.23 $\pm$ 0.03 & -23.41 $\pm$ 0.05 &  -6.96 $\pm$ 1.02 & -14.69 $\pm$ 0.29 & -10.27 $\pm$ 0.56\\
%   193 & 20333759-2556521 & M4.5 & -5.40 $\pm$ 0.95 & 13.1 & 34.55 $\pm$ 0.17 &  11.39 $\pm$ 0.06 & -23.62 $\pm$ 0.12 &  -8.44 $\pm$ 0.76 & -14.85 $\pm$ 0.26 &  -9.59 $\pm$ 0.52\\
%   205 & 21100535-1919573 & M2   & -6.34 $\pm$ 0.41 & 10.8 & 21.87 $\pm$ 0.06 &  12.25 $\pm$ 0.04 & -20.26 $\pm$ 0.06 &  -9.91 $\pm$ 0.28 & -15.17 $\pm$ 0.16 &  -9.78 $\pm$ 0.26\\
%   215 & 22424896-7142211 & K7   &  8.06 $\pm$ 0.15 &  9.8 & 19.57 $\pm$ 0.02 & -18.94 $\pm$ 0.02 & -24.54 $\pm$ 0.02 & -10.25 $\pm$ 0.08 & -15.84 $\pm$ 0.08 &  -7.98 $\pm$ 0.10\\
% \hline
% \hline
% \end{tabular}

% \end{sidewaystable*}{}


==> Tables/82_radial_velocities.tex <==
\newcolumntype{M}{>{\begin{varwidth}{2.5cm}}l<{\end{varwidth}}} %M is for Maximal column
\longtab{
\setlength{\tabcolsep}{4pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{longtable}{|M|r|M|M|M|M|r@{$\pm$}l|l|l|}
\caption{\label{tab:RV} Radial velocities measured in this study. Columns indicate: (1) 2MASS source ID; (2) number of spectra used to measure the radial velocity; (3) spectrograph; (4--6) radial velocity, radial velocity error and julian day of individual measures; (7) radial velocity; (8) binary flag (from literature), the asterisk indicates the binaries identified in this work; (9) contamination flag (see App.~\ref{App:discarded}). This file will be available at the CDS.}\\

\hline\hline
  \multicolumn{1}{|c|}{2MASS ID} &
  \multicolumn{1}{c|}{$n$} & %nSpecRV
  \multicolumn{1}{c|}{Instrument} & %refAP
  \multicolumn{1}{c|}{all RV} &
  \multicolumn{1}{c|}{all RV error} &
  \multicolumn{1}{c|}{all JD} &
  \multicolumn{2}{c|}{final RV} &
  \multicolumn{1}{c|}{Bin.} &
  \multicolumn{1}{c|}{Cont.} \\
  
  \multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{} & %nSpecRV
  \multicolumn{1}{c|}{} & %refAP
  \multicolumn{1}{c|}{(km~s$^{-1}$)} &
  \multicolumn{1}{c|}{(km~s$^{-1}$)} &
  \multicolumn{1}{c|}{(days)} &
  \multicolumn{2}{c|}{(km~s$^{-1}$)} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
  \multicolumn{1}{|c|}{2MASS ID} &
  \multicolumn{1}{c|}{$n$} & %nSpecRV
  \multicolumn{1}{c|}{Instrument} & %refAP
  \multicolumn{1}{c|}{all RV} &
  \multicolumn{1}{c|}{all RV error} &
  \multicolumn{1}{c|}{all JD} &
  \multicolumn{2}{c|}{final RV} &
  \multicolumn{1}{c|}{Bin.} &
  \multicolumn{1}{c|}{Cont.} \\
  
  \multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{} & %nSpecRV
  \multicolumn{1}{c|}{} & %refAP
  \multicolumn{1}{c|}{(km~s$^{-1}$)} &
  \multicolumn{1}{c|}{(km~s$^{-1}$)} &
  \multicolumn{1}{c|}{(days)} &
  \multicolumn{2}{c|}{(km~s$^{-1}$)} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\
\hline
\endhead
\hline\hline
\endfoot
  \object{J00172353-6645124} & 2 & FEROS & [10.38, 10.72] & [0.07, 0.07] & [2456286.53009, 2458691.92089] & 10.55 & 0.29 & N & N\\
  \object{J00275023-3233060} & 1 & FEROS & [8.75] & [0.07] & [2458689.82083] & 8.75 & 0.22 & Y & N\\
  \object{J00275035-3233238} & 1 & FEROS & [9.48] & [0.11] & [2458689.8417] & 9.48 & 0.27 & Y & N\\
  \object{J01365516-0647379} & 1 & FEROS & [13.02] & [0.18] & [2458690.90001] & 13.02 & 0.18 & N & Y\\
  \object{J01373545-0645375} & 1 & HARPS & [12.01] & [0.02] & [2456844.93243] & 12.01 & 0.12 & N & Y\\
  \object{J01535076-1459503} & 2 & FEROS & [11.24, 11.26] & [0.11, 0.1] & [2456486.94905, 2456486.9415] & 11.25 & 0.17 & Y & N\\
  \object{J02172472+2844305} & 9 & ELODIE + SOPHIE + UVES & [5.27, 5.42, 5.23, 5.29, 5.28, 5.34, 5.3, 5.28, 5.26] & [0.08, 0.07, 0.06, 0.07, 0.07, 0.07, 0.06, 0.06, 0.06] & [2453393.27103, 2454805.65735, 2454435.43376, 2456218.5035099997, 2454046.46631, 2454496.31713, 2454493.34131, 2456252.46093, 2454048.5668200003] & 5.3 & 0.17 & Y & N\\
  \object{J02232663+2244069} & 1 & FEROS & [12.6] & [0.04] & [2458697.90061] & 12.6 & 0.15 & N & Y\\
  \object{J02272804+3058405} & 3 & SOPHIE + UVES & [4.95, 4.9, 5.08] & [0.12, 0.12, 0.16] & [2458012.53643, 2457276.80723, 2458011.6425] & 4.98 & 0.22 & Y & N\\
  \object{J02272924+3058246} & 12 & SOPHIE + UVES & [6.14, 5.82, 6.15, 6.2, 6.04, 6.14, 6.04, 6.14, 6.07, 6.04, 6.15, 6.13] & [0.04, 0.04, 0.03, 0.04, 0.04, 0.03, 0.03, 0.03, 0.04, 0.03, 0.03, 0.04] & [2457234.61374, 2457276.81306, 2457240.6175, 2457301.53285, 2457236.55989, 2457239.6126200003, 2457237.61755, 2457239.6239400003, 2457236.5712099997, 2457237.62886, 2457240.60619, 2457234.62505] & 6.09 & 0.18 & Y & N\\
  \object{J03573393+2445106} & 3 & SOPHIE & [13.46, 13.44, 15.3] & [0.08, 0.08, 0.13] & [2458342.6218, 2458344.57798, 2458817.66093] & 14.07 & 1.0 & N & Y\\
  \object{J04373746-0229282} & 2 & FEROS + HARPS & [23.26, 23.86] & [0.09, 0.07] & [2457059.59525, 2456707.52487] & 23.56 & 0.39 & Y & N\\
  \object{J04593483+0147007} & 6 & UVES + HARPS & [19.74, 19.17, 19.21, 18.73, 19.33, 18.36] & [0.1, 0.11, 0.12, 0.11, 0.12, 0.13] & [2456987.719, 2455925.73967, 2457668.8121599997, 2452605.79882, 2457667.80028, 2454808.60375] & 19.09 & 0.53 & N & N\\
  \object{J05004714-5715255} & 1 & HARPS & [19.24] & [0.05] & [2453432.5492] & 19.24 & 0.19 & N & N\\
  \object{J05004928+1527006} & 3 & SOPHIE & [18.34, 18.71, 18.17] & [0.16, 0.19, 0.15] & [2454083.63576, 2454084.53989, 2454083.6129900003] & 18.41 & 0.33 & N & Y\\
  \object{J05015881+0958587} & 23 & ELODIE + UVES & [5.06, 18.47, 17.7, 24.22, 21.78, 24.55, 25.16, 23.09, 21.25, 16.64, 15.16, 22.26, 23.79, 7.01, 23.44, 24.37, 22.4, 5.29, 5.76, 7.24, 24.22, 24.82, 12.25] & [0.13, 0.2, 0.13, 0.16, 0.16, 0.13, 0.16, 0.15, 0.18, 0.16, 0.18, 0.22, 0.15, 0.17, 0.15, 0.16, 0.15, 0.16, 0.14, 0.14, 0.15, 0.15, 0.14] & [2450851.30098, 2457295.80643, 2452212.44015, 2450747.48517, 2450746.5646900004, 2451108.6050400003, 2450389.5120599996, 2451452.65497, 2450524.31012, 2450418.46055, 2450837.3486200003, 2452294.31977, 2450020.5901, 2450804.39026, 2450523.30293, 2450747.... & 18.08 & 8.68 & Y & N\\
  \object{J05064946-2135038} & 3 & UVES + HARPS & [22.63, 22.19, 22.12] & [0.04, 0.06, 0.06] & [2456305.6341, 2455846.7513599996, 2455847.76613] & 22.31 & 0.3 & Y & N\\
  \object{J05064991-2135091} & 2 & UVES + HARPS & [21.77, 21.18] & [0.04, 0.06] & [2456302.6532400004, 2455855.85902] & 21.48 & 0.36 & Y & N\\
  \object{J05320450-0305291} & 1 & UVES & [24.98] & [0.18] & [2455846.78251] & 24.98 & 0.24 & Y & N\\
  \object{J05332802-4257205} & 2 & FEROS & [1.79, -5.14] & [0.14, 0.08] & [2456559.88043, 2458698.87244] & -1.67 & 3.61 & Y & N\\
  \object{J05471708-5103594} & 6 & FEROS & [18.67, 19.09, 19.74, 19.0, 22.36, 20.55] & [3.54, 1.18, 1.25, 2.87, 1.06, 1.79] & [2456605.8494, 2456605.86038, 2456605.8580400003, 2456605.85157, 2456605.86272, 2456605.8552099997] & 19.92 & 5.49 & N & N\\
  \object{J06131330-2742054} & 2 & FEROS & [22.77, 22.83] & [0.04, 0.04] & [2456168.91567, 2456339.5863] & 22.8 & 0.23 & Y & N\\
  \object{J06182824-7202416} & 2 & UVES & [16.75, 15.72] & [0.28, 0.28] & [2455855.8541200003, 2454805.67937] & 16.24 & 0.71 & N & N\\
  \object{J08475676-7854532} & 1 & UVES & [23.12] & [0.15] & [2455932.80613] & 23.12 & 0.32 & N & Y\\
  \object{J10141918+2104297} & 9 & ELODIE + SOPHIE & [18.26, 22.14, 2.4, 22.11, 22.12, 15.16, 20.02, 21.87, 4.2] & [0.15, 0.1, 0.14, 0.1, 0.1, 0.1, 0.11, 0.09, 0.1] & [2450590.8267900003, 2454506.50303, 2451565.59044, 2454507.50358, 2454505.49547, 2454522.50716, 2454514.42432, 2454502.5578099997, 2454538.46624] & 16.48 & 8.99 & Y & N\\
  \object{J10172689-5354265} & 5 & FEROS + UVES + HARPS & [14.13, 13.97, 14.4, 14.71, 15.09] & [0.15, 0.16, 0.14, 0.13, 0.14] & [2455933.81672, 2457060.72187, 2454531.6129799997, 2457854.70352, 2454186.62003] & 14.46 & 0.76 & Y & N\\
  \object{J11493184-7851011} & 2 & FEROS + UVES & [15.15, 13.84] & [0.12, 0.08] & [2456808.54193, 2455935.81112] & 14.5 & 0.79 & N & Y\\
  \object{J13545390-7121476} & 1 & FEROS & [5.82] & [0.04] & [2458692.4826] & 5.82 & 0.21 & N & Y\\
  \object{J14423039-6458305} & 76 & FEROS + UVES + HARPS & [7.15, 6.64, 6.45, 7.21, 7.04, 6.48, 6.52, 7.57, 6.99, 7.08, 7.55, 7.08, 7.05, 7.07, 6.53, 7.15, 7.6, 7.66, 6.62, 7.53, 7.03, 6.76, 7.67, 6.45, 7.44, 7.54, 7.56, 7.13, 7.6, 6.61, 7.68, 7.05, 6.61, 7.15, 6.51, 7.0, 6.83, 7.55, 7.07, 7.53, 6.54, 6.78, 6.5... & [0.51, 0.72, 0.68, 0.84, 0.54, 0.7, 0.67, 0.72, 0.62, 0.49, 0.77, 0.62, 0.53, 0.57, 0.62, 0.62, 0.6, 0.61, 0.72, 0.75, 0.56, 0.56, 0.68, 0.68, 0.65, 0.62, 0.82, 0.6, 0.72, 0.73, 0.68, 0.6, 0.66, 0.67, 0.7, 0.59, 0.85, 0.72, 0.67, 0.6, 0.67, 0.59, 0.69, ... & [2456743.75264, 2454516.81487, 2454516.85847, 2453395.89146, 2454575.67859, 2454516.85069, 2454516.84632, 2454519.81322, 2454576.68172, 2454576.70225, 2454519.8244, 2454576.67895, 2454575.69137, 2454575.69965, 2454516.84253, 2454576.6929099998, 2454573.... & 7.09 & 0.79 & Y & N\\
  \object{J15385679-5742190} & 1 & FEROS & [-1.38] & [0.22] & [2457953.55469] & -1.38 & 0.25 & Y & N\\
  \object{J15385757-5742273} & 6 & FEROS + UVES & [-0.16, -1.4, 5.61, 5.51, 5.7, 6.76] & [0.29, 0.21, 0.23, 0.24, 0.23, 0.2] & [2454906.81955, 2456409.58371, 2456111.60845, 2456033.88833, 2456121.63853, 2455991.79432] & 3.67 & 3.67 & Y & N\\
  \object{J16120516-4556242} & 1 & FEROS & [19.92] & [0.09] & [2458698.51885] & 19.92 & 0.39 & N & Y\\
  \object{J16572029-5343316} & 1 & FEROS & [1.42] & [0.04] & [2458689.5540299998] & 1.42 & 0.16 & N & N\\
  \object{J17020937-6734447} & 1 & FEROS & [5.59] & [0.19] & [2458693.53133] & 5.59 & 0.93 & N & N\\
  \object{J17024014-4521587} & 1 & FEROS & [-2.63] & [0.06] & [2458689.53028] & -2.63 & 0.18 & N & N\\
  \object{J17092947-5235197} & 1 & FEROS & [-4.66] & [0.1] & [2458698.56121] & -4.66 & 0.16 & N & Y\\
  \object{J17172550-6657039} & 1 & FEROS & [-52.76] & [1.59] & [2457953.74579] & -52.76 & 1.64 & Y & N\\
  \object{J17173128-6657055} & 1 & FEROS & [4.22] & [0.05] & [2456912.51433] & 4.22 & 0.4 & Y & N\\
  \object{J17444256-5315471} & 1 & FEROS & [1.59] & [0.11] & [2458697.67149] & 1.59 & 0.38 & N & N\\
  \object{J17483374-5306118} & 1 & FEROS & [1.04] & [0.05] & [2458693.60248] & 1.04 & 0.13 & N & N\\
  \object{J18030341-5138564} & 2 & HARPS & [0.42, -0.15] & [0.24, 0.22] & [2457601.50675, 2457601.50292] & 0.14 & 0.55 & Y & N\\
  \object{J18030409-5138561} & 1 & FEROS & [0.93] & [0.62] & [2457317.52232] & 0.93 & 0.62 & Y & N\\
  \object{J18041617-3018280} & 1 & FEROS & [-7.41] & [0.09] & [2458690.6403200002] & -7.41 & 0.24 & N & N\\
  \object{J18055491-5704307} & 1 & FEROS & [0.65] & [0.09] & [2458691.6113400003] & 0.65 & 0.21 & N & N\\
  \object{J18092970-5430532} & 1 & FEROS & [-1.85] & [0.27] & [2458698.61357] & -1.85 & 0.27 & N & N\\
  \object{J18141047-3247344} & 1 & UVES & [-51.01] & [0.45] & [2452381.8705] & -51.01 & 0.59 & Y & N\\
  \object{J18161236-5844055} & 1 & FEROS & [3.22] & [0.38] & [2458692.52196] & 3.22 & 0.41 & N & N\\
  \object{J18281651-4421477} & 1 & FEROS & [-1.56] & [0.07] & [2458693.7825700003] & -1.56 & 0.23 & N & N\\
  \object{J18283524-4457280} & 1 & FEROS & [-1.02] & [0.05] & [2458689.66396] & -1.02 & 0.34 & N & N\\
  \object{J18420694-5554254} & 2 & FEROS & [0.4, 0.53] & [0.07, 0.12] & [2458694.59473, 2456807.79726] & 0.47 & 0.21 & N & N\\
  \object{J18430597-4058047} & 1 & FEROS & [3.92] & [0.24] & [2458692.6521] & 3.92 & 0.33 & N & Y\\
  \object{J18452691-6452165} & 3 & FEROS + HARPS & [-19.09, -18.92, 8.27] & [8.58, 1.63, 1.73] & [2454942.8009, 2457848.7899, 2457847.79691] & -9.87 & 18.89 & Y & N\\
  \object{J18530587-5010499} & 5 & FEROS & [-1.26, -2.49, -4.54, -5.0, -1.27] & [1.37, 1.97, 1.51, 3.47, 1.72] & [2456148.56861, 2456150.503, 2456148.60928, 2456148.55643, 2456147.62828] & -2.9 & 2.62 & Y & N\\
  \object{J19225894-5432170} & 6 & FEROS + UVES + HARPS & [0.15, 0.02, -0.11, -0.08, 0.2, 0.11] & [0.31, 0.38, 0.34, 0.35, 0.3, 0.35] & [2457849.83819, 2454943.7609200003, 2455850.5671599996, 2457492.81417, 2455035.6650799997, 2457590.58281] & 0.05 & 0.39 & N & N\\
  \object{J19233820-4606316} & 1 & FEROS & [0.08] & [0.15] & [2458689.7661] & 0.08 & 0.83 & N & N\\
  \object{J19243494-3442392} & 1 & FEROS & [-6.56] & [0.37] & [2458698.72299] & -6.56 & 0.63 & N & N\\
  \object{J19312434-2134226} & 1 & FEROS & [-36.59] & [0.39] & [2458689.70766] & -36.59 & 1.79 & Y$^{*}$ & N\\
  \object{J19481651-2720319} & 1 & FEROS & [-6.26] & [0.04] & [2458692.82234] & -6.26 & 0.16 & N & N\\
  \object{J19560294-3207186} & 3 & FEROS & [-41.2, -41.1, -41.18] & [0.09, 0.09, 0.08] & [2456204.5682099997, 2456204.57578, 2456204.5455400003] & -41.16 & 0.25 & Y & N\\
  \object{J19560438-3207376} & 2 & UVES & [-5.59, -6.02] & [0.05, 0.05] & [2457255.79898, 2455850.57303] & -5.8 & 0.3 & Y & N\\
  \object{J20013718-3313139} & 1 & UVES & [-4.27] & [0.05] & [2455850.58] & -4.27 & 0.19 & N & N\\
  \object{J20090521-2613265} & 2 & UVES & [-3.9, -5.53] & [0.51, 0.58] & [2455850.58564, 2455843.60407] & -4.71 & 1.2 & N & N\\
  \object{J20100002-2801410} & 1 & FEROS & [-6.75] & [0.68] & [2456560.53069] & -6.75 & 3.78 & Y & N\\
  \object{J20105054-3844326} & 1 & FEROS & [-10.34] & [0.04] & [2458690.79121] & -10.34 & 0.2 & N & Y\\
  \object{J20333759-2556521} & 1 & FEROS & [-5.4] & [0.21] & [2458695.78175] & -5.4 & 0.95 & N & N\\
  \object{J20415111-3226073} & 1 & HARPS & [-3.17] & [0.48] & [2453467.92167] & -3.17 & 0.53 & Y & N\\
  \object{J20450949-3120266} & 2 & HARPS & [-4.28, -4.57] & [0.1, 0.1] & [2456844.8056400004, 2453551.79857] & -4.42 & 0.22 & Y & N\\
  \object{J21100535-1919573} & 2 & FEROS & [-6.66, -6.03] & [0.16, 0.15] & [2458694.7842, 2456558.58511] & -6.34 & 0.41 & N & N\\
  \object{J21212873-6655063} & 1 & FEROS & [2.98] & [0.04] & [2456204.70163] & 2.98 & 0.32 & N & Y\\
  \object{J22424896-7142211} & 2 & UVES & [8.07, 8.04] & [0.05, 0.05] & [2454765.5580700003, 2454765.55583] & 8.06 & 0.15 & N & N\\
  \object{J22445794-3315015} & 1 & UVES & [2.23] & [0.53] & [2455850.59465] & 2.23 & 0.62 & Y & N\\
  \object{J22450004-3315258} & 1 & UVES & [3.12] & [0.93] & [2455850.60316] & 3.12 & 0.95 & Y & N\\
  \object{J23172807+1936469} & 11 & ELODIE + SOPHIE & [-1.95, -2.19, -1.11, 1.15, -1.57, -1.77, 6.36, -2.16, -2.25, -2.08, -1.18] & [0.19, 0.35, 0.14, 0.17, 0.13, 0.12, 0.17, 0.13, 0.22, 0.13, 0.12] & [2453630.46255, 2454035.3979700003, 2452844.49411, 2452544.50705, 2452929.38462, 2454383.45849, 2452157.44928, 2453229.5270599998, 2453597.5269299997, 2453266.51664, 2452840.58586] & -0.79 & 1.5 & Y & N\\
  \object{J23301341-2023271} & 1 & FEROS & [-18.68] & [0.07] & [2456202.60367] & -18.68 & 0.2 & Y & N\\
  \object{J23314492-0244395} & 1 & FEROS & [-4.97] & [0.06] & [2458690.82999] & -4.97 & 0.31 & N & Y\\
  \object{J23512227+2344207} & 1 & FEROS & [-0.97] & [0.06] & [2458697.76885] & -0.97 & 0.3 & N & Y\\
  \object{J00323480+0729271} & 6 & SOPHIE + CAFE & [-4.35, -4.64, -4.85, -2.26, -0.76, -1.69] & [0.82, 0.58, 0.78, 0.73, 0.72, 0.76] & [2458341.5348099996, 2458390.460536357, 2458341.55666, 2458342.53059, 2458346.52207, 2458346.54459] & -3.09 & 1.96 & Y & N\\
  \object{J21183375+3014346} & 7 & SOPHIE + CAFE & [-21.77, -22.1, -21.83, -22.14, -21.61, -22.36, -22.2] & [0.05, 0.07, 0.04, 0.07, 0.04, 0.08, 0.07] & [2458317.527562027, 2458341.49193, 2458317.549529868, 2458342.4811299997, 2458317.5725100595, 2458343.46208, 2458344.48195] & -22.0 & 0.32 & N & Y\\
  \object{J21374019+0137137} & 1 & CAFE & [-18.26] & [0.15] & [2458387.38651578] & -18.26 & 0.38 & Y & N\\
  \object{J22184265+3321137} & 8 & SOPHIE + CAFE & [8.69, -19.51, 5.41, 8.33, -0.27, -18.33, 5.37, -23.64] & [0.08, 0.1, 0.16, 0.1, 0.16, 0.16, 0.09, 0.19] & [2458324.634014213, 2458668.57474, 2458341.50504, 2458324.6780905467, 2458342.4928900003, 2458344.51913, 2458387.400183964, 2458345.53959] & -4.24 & 14.04 & Y & N\\
  \object{J22571130+3639451} & 8 & SOPHIE + CAFE & [-14.02, -17.09, -9.88, -16.44, -15.11, -18.51, -16.05, -15.85] & [0.13, 0.26, 0.19, 0.92, 0.22, 0.17, 0.28, 0.21] & [2458317.6042934787, 2458341.51765, 2458317.6262624767, 2458342.50408, 2458317.648227424, 2458317.6703799074, 2458344.53684, 2458391.458978862] & -15.36 & 1.75 & Y$^{*}$ & N\\
\end{longtable}
}

% \longtab{
% \begin{longtable}{|r|l|r|l|r@{$\pm$}l|l|l|l|}
% \caption{\label{tab:RV} Radial velocities measured in this study. Columns indicate: (1) 2MASS source ID; (2) number of spectra used to measure the radial velocity; (3) spectrograph; (4) radial veloscity; (5) binary flag (from literature), the asterisk indicates the binaries identified in this work; (6) 6D data flag, indicates if the source has \textit{Gaia} DR2 astrometry; (7) contamination flag. \nm{Remove internal ID}}\\
% % \begin{tabular}{|r|l|r|l|r@{$\pm$}l|l|l|l|}
% \hline\hline
%   \multicolumn{1}{|c|}{SourceID} &
%   \multicolumn{1}{c|}{2MASS ID} &
%   \multicolumn{1}{c|}{nSpec} & %nSpecRV
%   \multicolumn{1}{c|}{Instrument} & %refAP
%   \multicolumn{2}{c|}{RV (km~s$^{-1}$)} &
%   \multicolumn{1}{c|}{Bin.} &
%   \multicolumn{1}{c|}{6D} &
%   \multicolumn{1}{c|}{Cont.} \\
% \hline
% \endfirsthead
% \caption{continued.}\\
% \hline\hline
%   \multicolumn{1}{|c|}{SourceID} &
%   \multicolumn{1}{c|}{2MASS ID} &
%   \multicolumn{1}{c|}{nSpec} & %nSpecRV
%   \multicolumn{1}{c|}{Instrument} & %refAP
%   \multicolumn{2}{c|}{RV (km~s$^{-1}$)} &
%   \multicolumn{1}{c|}{Bin.} &
%   \multicolumn{1}{c|}{6D} &
%   \multicolumn{1}{c|}{Cont.} \\
% \hline
% \endhead
% \hline\hline
% \endfoot
%     4 & \object{2MASS J00172353-6645124} &  2 & FEROS              &   10.55 &  0.29 & N       & Y & N\\
%     6 & \object{2MASS J00275023-3233060} &  1 & FEROS              &    8.75 &  0.22 & Y       & Y & N\\
%     7 & \object{2MASS J00275035-3233238} &  1 & FEROS              &    9.48 &  0.27 & Y       & Y & N\\
%   17 & \object{2MASS J01365516-0647379} &  1 & FEROS              &   13.02 &  0.18 & N       & Y & N\\
%   18 & \object{2MASS J01373545-0645375} &  1 & HARPS              &   12.01 &  0.12 & N       & Y & Y\\
%   21 & \object{2MASS J01535076-1459503} &  2 & FEROS              &   11.25 &  0.17 & Y       & N & N\\
%   23 & \object{2MASS J02172472+2844305} &  9 & ELODIE+SOPHIE+UVES &    5.3  &  0.17 & Y       & Y & N\\
%   27 & \object{2MASS J02232663+2244069} &  1 & FEROS              &   12.60 &  0.15 & N       & Y & Y\\
%   29 & \object{2MASS J02272804+3058405} &  3 & SOPHIE+UVES        &    4.98 &  0.22 & Y       & Y & N\\
%   30 & \object{2MASS J02272924+3058246} & 12 & SOPHIE+UVES        &    6.09 &  0.18 & Y       & Y & N\\
%   45 & \object{2MASS J03573393+2445106} &  3 & SOPHIE             &   14.07 &  1.0  & Y$^{*}$ & Y & N\\
%   54 & \object{2MASS J04373746-0229282} &  2 & FEROS+HARPS        &   23.56 &  0.39 & Y       & N & N\\
%   60 & \object{2MASS J04593483+0147007} &  6 & UVES+HARPS         &   19.09 &  0.53 & N       & Y & N\\
%   61 & \object{2MASS J05004714-5715255} &  1 & HARPS              &   19.24 &  0.19 & N       & Y & N\\
%   62 & \object{2MASS J05004928+1527006} &  3 & SOPHIE             &   18.41 &  0.33 & N       & Y & Y\\
%   63 & \object{2MASS J05015881+0958587} & 23 & ELODIE+UVES        &   18.08 &  8.68 & Y       & Y & N\\
%   65 & \object{2MASS J05064946-2135038} &  3 & UVES+HARPS         &   22.31 &  0.3  & Y       & N & N\\
%   66 & \object{2MASS J05064991-2135091} &  2 & UVES+HARPS         &   21.48 &  0.36 & Y       & Y & N\\
%   76 & \object{2MASS J05320450-0305291} &  1 & UVES               &   24.98 &  0.24 & Y       & N & N\\
%   77 & \object{2MASS J05332802-4257205} &  2 & FEROS              &   -1.67 &  3.61 & Y       & Y & N\\
%   82 & \object{2MASS J05471708-5103594} &  6 & FEROS              &   19.92 &  5.49 & N       & Y & N\\
%   84 & \object{2MASS J06131330-2742054} &  2 & FEROS              &   22.8  &  0.23 & Y       & Y & N\\
%   87 & \object{2MASS J06182824-7202416} &  2 & UVES               &   16.24 &  0.71 & N       & Y & N\\
%   93 & \object{2MASS J08475676-7854532} &  1 & UVES               &   23.12 &  0.32 & N       & Y & Y\\
%   95 & \object{2MASS J10141918+2104297} &  9 & ELODIE+SOPHIE      &   16.48 &  8.99 & Y       & N & N\\
%   96 & \object{2MASS J10172689-5354265} &  5 & FEROS+UVES         &   14.46 &  0.76 & Y       & Y & N\\
%   97 & \object{2MASS J11493184-7851011} &  2 & FEROS+UVES         &   14.5  &  0.79 & N       & Y & Y\\
%   98 & \object{2MASS J13545390-7121476} &  1 & FEROS              &   5.82  &  0.21 & N       & Y & Y\\
%   100 & \object{2MASS J14423039-6458305} & 76 & FEROS+UVES+HARPS   &   7.09  &  0.79 & Y       & Y & N\\
%   101 & \object{2MASS J15385679-5742190} &  1 & FEROS              &   -1.38 &  0.25 & Y       & Y & N\\
%   102 & \object{2MASS J15385757-5742273} &  6 & FEROS+UVES         &    3.67 &  3.67 & Y       & Y & N\\
%   103 & \object{2MASS J16120516-4556242} &  1 & FEROS              &   19.92 &  0.39 & N       & Y & Y\\
%   104 & \object{2MASS J16181789-2836502} & 36 & HARPS              &  -12.53 &  4.91 & N       & Y & N\\
%   107 & \object{2MASS J16572029-5343316} &  1 & FEROS              &    1.42 &  0.16 & N       & Y & N\\
%   109 & \object{2MASS J17020937-6734447} &  1 & FEROS              &    5.59 &  0.93 & N       & Y & N\\
%   111 & \object{2MASS J17024014-4521587} &  1 & FEROS              &   -2.63 &  0.18 & N       & Y & N\\
%   112 & \object{2MASS J17092947-5235197} &  1 & FEROS              &   -4.66 &  0.16 & N       & Y & Y\\
%   114 & \object{2MASS J17172550-6657039} &  1 & FEROS              &  -52.76 &  1.64 & Y       & Y & N\\
%   115 & \object{2MASS J17173128-6657055} &  1 & FEROS              &    4.22 &  0.4  & Y       & Y & N\\
%   120 & \object{2MASS J17444256-5315471} &  1 & FEROS              &    1.59 &  0.38 & N       & Y & N\\
%   122 & \object{2MASS J17483374-5306118} &  1 & FEROS              &    1.04 &  0.13 & N       & Y & N\\
%   124 & \object{2MASS J18030341-5138564} &  2 & HARPS              &    0.14 &  0.55 & Y       & Y & N\\
%   125 & \object{2MASS J18030409-5138561} &  1 & FEROS              &    0.93 &  0.62 & Y       & Y & N\\
%   127 & \object{2MASS J18041617-3018280} &  1 & FEROS              &   -7.41 &  0.24 & N       & Y & N\\
%   128 & \object{2MASS J18055491-5704307} &  1 & FEROS              &    0.65 &  0.21 & N       & Y & N\\
%   131 & \object{2MASS J18092970-5430532} &  1 & FEROS              &   -1.85 &  0.27 & N       & Y & N\\
%   133 & \object{2MASS J18141047-3247344} &  1 & UVES               &  -51.01 &  0.59 & Y       & Y & N\\
%   137 & \object{2MASS J18161236-5844055} &  1 & FEROS              &    3.22 &  0.41 & N       & Y & N\\
%   142 & \object{2MASS J18281651-4421477} &  1 & FEROS              &   -1.56 &  0.23 & N       & Y & N\\
%   144 & \object{2MASS J18283524-4457280} &  1 & FEROS              &   -1.02 &  0.34 & N       & Y & N\\
%   146 & \object{2MASS J18420694-5554254} &  2 & FEROS              &    0.47 &  0.21 & N       & Y & N\\
%   147 & \object{2MASS J18430597-4058047} &  1 & FEROS              &    3.92 &  0.33 & N       & Y & Y\\
%   148 & \object{2MASS J18452691-6452165} &  3 & FEROS+HARPS        &   -9.87 & 18.89 & Y       & Y & N\\
%   154 & \object{2MASS J18530587-5010499} &  5 & FEROS              &    -2.9 &  2.62 & Y       & Y & N\\
%   167 & \object{2MASS J19225894-5432170} &  6 & UVES+HARPS         &    0.05 &  0.39 & N       & Y & N\\
%   168 & \object{2MASS J19233820-4606316} &  1 & FEROS              &    0.08 &  0.83 & N       & Y & N\\
%   169 & \object{2MASS J19243494-3442392} &  1 & FEROS              &   -6.56 &  0.63 & N       & Y & N\\
%   174 & \object{2MASS J19312434-2134226} &  1 & FEROS              &  -36.59 &  1.79 & Y$^{*}$ & Y & N\\
%   178 & \object{2MASS J19481651-2720319} &  1 & FEROS              &   -6.26 &  0.16 & N       & Y & N\\
%   181 & \object{2MASS J19560294-3207186} &  3 & FEROS              &  -41.16 &  0.25 & Y       & Y & N\\
%   182 & \object{2MASS J19560438-3207376} &  2 & UVES               &    -5.8 &  0.3  & Y       & Y & N\\
%   184 & \object{2MASS J20013718-3313139} &  1 & UVES               &   -4.27 &  0.19 & N       & Y & N\\
%   187 & \object{2MASS J20090521-2613265} &  2 & UVES               &   -4.71 &  1.2  & N       & Y & N\\
%   188 & \object{2MASS J20100002-2801410} &  1 & FEROS              &   -6.75 &  3.78 & Y       & N & N\\
%   189 & \object{2MASS J20105054-3844326} &  1 & FEROS              &  -10.34 &  0.2  & N       & Y & Y\\
%   193 & \object{2MASS J20333759-2556521} &  1 & FEROS              &    -5.4 &  0.95 & N       & Y & N\\
%   195 & \object{2MASS J20415111-3226073} &  1 & HARPS              &   -3.17 &  0.53 & Y       & N & N\\
%   199 & \object{2MASS J20450949-3120266} &  2 & HARPS              &   -4.42 &  0.22 & Y       & Y & N\\
%   205 & \object{2MASS J21100535-1919573} &  2 & FEROS              &   -6.34 &  0.41 & N       & Y & N\\
%   209 & \object{2MASS J21212873-6655063} &  1 & FEROS              &    2.98 &  0.32 & N       & Y & Y\\
%   215 & \object{2MASS J22424896-7142211} &  2 & UVES               &    8.06 &  0.15 & N       & Y & N\\
%   216 & \object{2MASS J22445794-3315015} &  1 & UVES               &    2.23 &  0.62 & Y       & Y & N\\
%   217 & \object{2MASS J22450004-3315258} &  1 & UVES               &    3.12 &  0.95 & Y       & Y & N\\
%   219 & \object{2MASS J23172807+1936469} & 11 & ELODIE+SOPHIE      &   -0.79 &  1.5  & Y       & N & N\\
%   222 & \object{2MASS J23301341-2023271} &  1 & FEROS              &  -18.68 &  0.2  & Y       & Y & N\\
%   223 & \object{2MASS J23314492-0244395} &  1 & FEROS              &   -4.97 &  0.31 & N       & Y & Y\\
%   229 & \object{2MASS J23512227+2344207} &  1 & FEROS              &   -0.97 &  0.3  & Y$^{*}$ & Y & N\\
%   230 & \object{2MASS J00323480+0729271} &  6 & SOPHIE+CAFE        &   -3.09 &  1.96 & Y       & N & N\\
%   231 & \object{2MASS J21183375+3014346} &  7 & SOPHIE+CAFE        &  -22.0  &  0.32 & N       & Y & Y\\
%   232 & \object{2MASS J21374019+0137137} &  1 & CAFE               &  -18.26 &  0.38 & Y       & N & N\\
%   233 & \object{2MASS J22184265+3321137} &  8 & SOPHIE+CAFE        &   -4.24 & 14.04 & Y       & Y & N\\
%   234 & \object{2MASS J22571130+3639451} &  8 & SOPHIE+CAFE        &  -15.36 &  1.75 & Y$^{*}$ & Y & N\\
% % \hline\end{tabular}
% \end{longtable}
% }




==> Tables/DA_diff_pots.tex <==
\begin{table*}
    \centering
    \caption{Dynamical age (in Myr) obtained with the robust metrics for different potentials. We report the mode and the highest density interval for probabilities of 68\%, 95\%, and 99.7\%.}
    \label{tab:DA_diff_pots}
\begin{tabular}{l|c|ccccccc}
\hline
\hline
 Potential & Size estimator & $p_{0.15}$ & $p_{2.5}$ & $p_{16}$ & mode & $p_{84}$ & $p_{97.5}$ & $p_{99.85}$ \\
\hline
new A\&S        & $S_{DCM}$ &   -32.0 &  -27.6 &  -21.1 &  -17.6 &  -14.7 &  -6.8 &    0 \\
McMillan17      & $S_{DCM}$ &   -43.9 &  -29.3 &  -20.2 &  -17.7 &  -14.6 &  -8.1 &    0 \\
MWPotential14   & $S_{DCM}$ &   -46.5 &  -27.8 &  -21.2 &  -17.7 &  -14.6 &  -6.1 &  -1.5 \\
\hline
new A\&S + spiral arms (P03) & $S_{DCM}$ &   -46.4 &  -29.3 &  -20.8 &  -17.9 &  -14.4 &  -7.6 &    0 \\
\hline
\hline
new A\&S        & $S_{TCM}$ &   -25.2 &  -22.0 &  -20.5 &  -18.5 &  -15.9 &  -5.6 &    0 \\
McMillan17      & $S_{TCM}$ &   -26.3 &  -22.2 &  -19.7 &  -18.2 &  -15.2 &  -8.6 &    0 \\
MWPotential14   & $S_{TCM}$ &   -26.3 &  -23.7 &  -20.7 &  -18.7 &  -16.2 &  -7.6 &    0 \\
\hline
new A\&S + spiral arms (P03) & $S_{TCM}$ &   -26.4 &  -22.3 &  -20.2 &  -18.5 &  -15.9 &  -5.6 &    0 \\
\hline
\hline
\end{tabular}
     
\end{table*}{}




% \begin{table*}
%     \centering
%     \caption{Dynamical age obtained with different potentials.}
%     \label{tab:DA_diff_pots}
% \begin{tabular}{l|ccccccc}
% \hline
% \hline
%  Potental & $p_{0.15}$ & $p_{2.5}$ & $p_{16}$ & $p_{50}$ & $p_{84}$ & $p_{97.5}$ & $p_{99.85}$ \\
% \hline
% \citet{Allen+91}    &   -47.6 &  -30.3 &  -20.9 &  -17.9 &  -14.1 &  -6.2 &    0.0 \\
% \citet{McMillan17}  &   -43.9 &  -28.3 &  -20.2 &  -17.7 &  -14.1 &  -7.6 &    0.0 \\
% \citet{Bovy15}      &   -46.2 &  -29.3 &  -21.2 &  -18.2 &  -14.1 &  -7.6 &    0.0 \\
% \hline
% \citet{Allen+91} + \citet{Pichardo03} &   -41.1 &  -29.4 &  -21.1 &  -17.9 &  -13.8 &  -6.2 &    0.0 \\
% \hline
% \hline
% \end{tabular}
     
% \end{table*}{}


==> Tables/age_review.tex <==
\begin{table*}
    \centering
    \caption{Literature age estimates for $\beta$~Pic. This table is an udated version of Table~1 from \citet{Mamajek14}.}
    \label{tab:age_review}
    \begin{tabular}{|l|c|l|}
        \hline
        \hline
        Reference               & Age                            & Method \\
        \hline
        \cite{Barrado99}        & $20\pm10$~Myr                  & CMD isochronal age (KM stars)\\
        \cite{Zuckerman+01}     & $12^{+8}_{-4}$~Myr             & H-R diagram isochronal age (KM stars)\\ % (GKM stars)+Li depletion \\
        \cite{Ortega02}         & $11.5$~Myr                     & Dynamical (Traceback) age \\              
        \cite{Song+03}          & $12$~Myr                       & Dynamical (Traceback) age \\     
        \cite{Ortega04}         & $10.8\pm0.3$~Myr               & Dynamical (Traceback) age \\
        \cite{Torres+06}        & $18$~Myr                       & Dynamical (Expansion) age \\             
        \cite{Makarov07}        & $31\pm21$~Myr                  & Dynamical (Traceback) age \\             
        \cite{Mentuch+08}       & $21\pm9$~Myr                   & Li depletion   \\               
        \cite{Macdonald+10}     & $\sim40$~Myr                   & Li depletion (magnetoconvection models) \\       
        \cite{Binks+14}         & $21\pm4$~Myr                   & Li depletion boundary   \\             
        \cite{Malo+14}          & $26\pm3$~Myr                   & Li depletion boundary   \\            
        \cite{Malo+14}          & $21.5\pm6.5$~Myr (15--28 Myr)  & H–R diagram isochronal age (KM stars)   \\ 
        \cite{Mamajek14}        & $22\pm3$~Myr                   & CMD isochronal age (FG stars)   \\     
        \cite{Mamajek14}        & $13-58$~Myr                    & Dynamical (Expansion) age   \\  
        \cite{Bell+2015}        & $24\pm3$~Myr                   & CMD isochronal age \\
        \cite{Messina+16}       & $25\pm3$~Myr                   & Li depletion boundary (rotation models) \\ 
        \cite{Miret-Roig+18}    & $13^{+7}_{-0}$~Myr             & Dynamical (Traceback) age   \\          
        \cite{Crundall+19}      & $18.3_{-1.2}^{+1.3}$~Myr       & Dynamical (Forward-modelling) age  \\ 
        \cite{Ujjwal+20}        & 19.38~Myr ($5.5-54.5$~Myr)     & CMD isochronal age \\
        \hline
        \textbf{This work} & \textbf{18.5$_{-2.4}^{+2.0}$~Myr} & \textbf{Dynamical (Traceback) age} \\
        \hline
        \hline
      
    \end{tabular}
\end{table*}{}


%   \begin{tabular}{|l|c|c|l|}
%         \hline
%         \hline
%         Reference               & Members  & Age                            & Method \\
%         \hline
%         \cite{Barrado99}        &   3 & $20\pm10$~Myr                  & CMD isochronal age (KM stars)\\
%         \cite{Zuckerman+01}     &  12 & $12^{+8}_{-4}$~Myr             & H-R diagram isochronal age (KM stars)\\ % (GKM stars)+Li depletion \\
%         \cite{Ortega02}         &  19 & $11.5$~Myr                     & Dynamical (Traceback) age \\              
%         \cite{Song+03}          &  24 & $12$~Myr                       & Dynamical (Traceback) age \\     
%         \cite{Ortega04}         &  14 & $10.8\pm0.3$~Myr               & Dynamical (Traceback) age \\
%         \cite{Torres+06}        &  41 & $18$~Myr                       & Dynamical (Expansion) age \\             
%         \cite{Makarov07}        &  17 & $31\pm21$~Myr                  & Dynamical (Traceback) age \\             
%         \cite{Mentuch+08}       &     & $21\pm9$~Myr                   & Li depletion   \\               
%         \cite{Macdonald+10}     &     & $\sim40$~Myr                   & Li depletion (magnetoconvection models) \\       
%         \cite{Binks+14}         &     & $21\pm4$~Myr                   & Li depletion boundary   \\             
%         \cite{Malo+14}          &     & $26\pm3$~Myr                   & Li depletion boundary   \\            
%         \cite{Malo+14}          &     & $21.5\pm6.5$~Myr (15--28 Myr)  & H–R diagram isochronal age (KM stars)   \\ 
%         \cite{Mamajek14}        &     & $22\pm3$~Myr                   & CMD isochronal age (FG stars)   \\     
%         \cite{Mamajek14}        &  30 & $13-58$~Myr                    & Dynamical (Expansion) age   \\             
%         \cite{Messina+16}       &     & $25\pm3$~Myr                   & Li depletion boundary (rotation models) \\ 
%         \cite{Miret-Roig+18}    &  21 & $13^{+7}_{-0}$~Myr             & Dynamical (Traceback) age   \\          
%         \cite{Crundall+19}      &  58 & $18.3_{-1.2}^{+1.3}$~Myr       & Dynamical (Forward-modelling) age  \\ 
%         % \cite{Ujjwal+20}        &     & $5.5-54.5$~Myr                 & CMD isochronal age \\
%         \hline
%         \textbf{This work} & \textbf{21} & \textbf{18$_{-4}^{+3}$~Myr} & \textbf{Dynamical (Traceback) age} \\
%         \hline
%         \hline
      
%     \end{tabular}


==> Tables/median_velocity.tex <==
% \begin{table}[]
%     \centering
%      \caption{Median heliocentric velocity and standard deviation of $\beta$~Pic measured with the final sample of 26 members.}
%     \label{tab:median_velocity}
%     \begin{tabular}{l|r}
%     \hline
%     \hline
%     $U$ (km~s$^{-1}$) & $-8.44$\\
%     $V$ (km~s$^{-1}$) & $-15.87$\\
%     $W$ (km~s$^{-1}$) & $-9.09$\\
%     \hline
%     $\sigma_{obs, U}$ (km~s$^{-1}$) & $1.57$\\
%     $\sigma_{obs, V}$ (km~s$^{-1}$) & $0.70$\\
%     $\sigma_{obs, W}$ (km~s$^{-1}$) & $0.74$\\
%     \hline
%     $\sigma_{err, U}$ (km~s$^{-1}$) & $0.24$\\
%     $\sigma_{err, V}$ (km~s$^{-1}$) & $0.12$\\
%     $\sigma_{err, W}$ (km~s$^{-1}$) & $0.12$\\
%     \hline
%     $\sigma_{int, U}$ (km~s$^{-1}$) & $1.55$\\
%     $\sigma_{int, V}$ (km~s$^{-1}$) & $0.69$\\
%     $\sigma_{int, W}$ (km~s$^{-1}$) & $0.73$\\
%     \hline
%     \hline
%     \end{tabular}
% \end{table}



\setlength{\tabcolsep}{7pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{table*}
    \centering
    \caption{Parameters of the distribution in positions (in pc) and in velocities (in km~s$^{-1}$) of the 26 bona fide kinematic members of $\beta$~Pic in the present ($t=0$~Myr). }
    \begin{tabular}{ccc|ccc|ccc|ccc}
    \hline
    \hline
   \multicolumn{12}{c}{Positions}\\
    \hline
    \hline
    $X$ & $Y$ & $Z$ & $\sigma_{obs, X}$ & $\sigma_{obs, Y}$ & $\sigma_{obs, Z}$ & $\sigma_{err, X}$ & $\sigma_{err, Y}$ & $\sigma_{err, Z}$ & $\sigma_{int, X}$ & $\sigma_{int, Y}$ & $\sigma_{int, Z}$\\
    \hline
   $47.49$ & $-7.89$ & $-17.92$ & $16.04$ & $13.18$ & $7.44$ & $0.11$ & $0.04$ & $0.05$ & $15.93$ & $13.14$ & $7.39$\\
   \hline
   \hline
   \multicolumn{12}{c}{Velocities}\\
    \hline
    \hline
    $U$ & $V$ & $W$ & $\sigma_{obs, U}$ & $\sigma_{obs, V}$ & $\sigma_{obs, W}$ & $\sigma_{err, U}$ & $\sigma_{err, V}$ & $\sigma_{err, W}$ & $\sigma_{int, U}$ & $\sigma_{int, V}$ & $\sigma_{int, W}$\\
    % (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) & (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$) &  (km~s$^{-1}$)\\
    \hline
    % $-8.44$ & $-15.87$ & $-9.09$ & $1.57$ & $0.70$ & $0.74$ & $0.24$ & $0.12$ & $0.12$ & $1.55$ & $0.69$ & $0.73$\\
   $-8.74$ & $-16.16$ & $-9.98$ & $1.49$ & $0.54$ & $0.70$ & $0.24$ & $0.11$ & $0.11$ & $1.25$ & $0.43$ & $0.59$\\
    \hline
    \hline
    \end{tabular}
    \tablefoot{Columns indicate: (1--3) central location of the distribution, (4--6) robust standard deviation, (7--9) median errors, and (10--12) a rough estimate of the intrinsic dispersion, computed as $\sigma_{int}^2 = \sigma_{obs}^2 - \sigma_{err}^2$.}

    \label{tab:median_velocity}
\end{table*}


==> Tables/num_source.tex <==
\begin{table*}
   \begin{center}
    \caption{Number of sources at each step of the data selection process (see Sect.~\ref{sec:data}).}
    \label{tab:num_sources}
    \begin{tabular}{lr|r|c|c|c}
    \hline
    \hline
    % \multicolumn{2}{l}{} &
    % \multicolumn{1}{|c|}{\# Members} &
    % \multicolumn{1}{c|}{Median} &
    % \multicolumn{1}{c|}{Median} & % and number of sources
    % \multicolumn{1}{c}{Median}\\
     \multicolumn{2}{l}{} &
    \multicolumn{1}{|c|}{\# Members} &
    \multicolumn{1}{c|}{ground-based RV error} &
    \multicolumn{1}{c|}{\textit{Gaia} RV error} & 
    \multicolumn{1}{c}{\textit{Gaia} $V_{tan}$ error}\\
   
    \multicolumn{2}{l}{} &
    \multicolumn{1}{|c|}{} &
    \multicolumn{1}{c|}{(km~s$^{-1}$)} &
    \multicolumn{1}{c|}{(km~s$^{-1}$)} &
    \multicolumn{1}{c}{(km~s$^{-1}$)}\\
    \hline
    \multicolumn{2}{l|}{Candidate members from literature}                         & 236 & 0.5$^*$ & 0.6~(55) & 0.19~(222) \\
    \hline                      
    \multicolumn{2}{l|}{High quality RV (this work)}                               &  81 & 0.3~~     & 0.6~(31) & 0.08~~~(79) \\
    \hline
    \multicolumn{2}{l|}{6D data (\textit{Gaia} astrometry + high quality RV)}      &  79 & 0.3~~     & 0.6~(31) & 0.08~~~~~~~~~ \\
    \multicolumn{1}{l}{\qquad Suspected SB (this work)} & \multicolumn{1}{r|}{2}   & & & &\\
    \multicolumn{1}{l}{\qquad SB from literature} &       \multicolumn{1}{r|}{35}  & & & &\\
    \multicolumn{1}{l}{\qquad Single} &                   \multicolumn{1}{r|}{42}  & & & &\\
    \hline 
    \multicolumn{2}{l|}{Single following kinematic criteria (see Sect.~\ref{subsec:vel_dist})}                      &  27 & \multirow{2}{*}{0.3~~} &  \multirow{2}{*}{0.6~(13)}  & \multirow{2}{*}{0.05~~~~~~~~~ } \\
    \multicolumn{2}{l|}{Confirmed by orbital analysis (bona fide sample)   }                         &  26 & & & \\
    \hline
    \hline
    \end{tabular}
    \end{center}{}
    \tablefoot{Columns 3--4 indicate the median radial velocity error obtained from ground-based surveys and from the \textit{Gaia} DR2 catalogue, respectively. For comparison, in column 5 we indicate the median tangential errors obtained with the \textit{Gaia} DR2 parallaxes and proper motions, obtained taking into account the correlation among the astrometric parameters. The number of \textit{Gaia} sources used to estimate the median velocity errors is indicated in brackets in each case.\\
    \noindent\tablefoottext{*}{median radial velocity errors published in the literature for the 137 stars with radial velocity previous to this work. This sample is inhomogeneous and may be affected by systematic errors among different studies.}} 

\end{table*}{}



% \begin{table}
%     \centering
%     \caption{Number of sources with different characteristics. The first five rows review the selection process followed to obtain the final sample used to study the dynamical age. The last four rows review the number of binaries and contaminants from the subset with 6D data. }
%     \label{tab:num_sources}
%     \begin{tabular}{l|r}
%     \hline
%     \hline
%     Compilation candidate members   &  236\\
%     RV from this work               &  82 \\
%     6D data                         &  72 \\
%     Singles literature              &  45 \\
%     Final sample this work          &  26 \\
%     \hline
%     Binaries                        & 31 \\
%     Singles                         & 26 \\
%     Contaminants                    & 13 \\
%     Poor radial velocity            &  2 \\
%     \hline
%     \hline
%     \end{tabular}
% \end{table}{}

==> Tables/spectra.tex <==
\begin{table} %[!h]
% \renewcommand\thetable{1} 
\centering
\caption{Spectra analysed in this study from our spectroscopic observations plus archival data. 
\label{tab:num-spectra}}
\begin{tabular}{lrr@{$-$}rr@{/}l}
\hline\hline
  \multicolumn{1}{c}{Spectrograph} &
  \multicolumn{1}{c}{$R$} & 
  \multicolumn{2}{c}{$\Delta\lambda$} & 
  \multicolumn{2}{c}{\# Spectra} \\
  
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} & 
  \multicolumn{2}{c}{(nm)} & 
  \multicolumn{2}{c}{total/this work} \\
%   \multicolumn{1}{c}{total} \
%   \multicolumn{1}{c}{this work} \\

% Spectrograph &$R$&$\Delta\lambda$&\# Spectra\\
% &&(nm)& total/this work\\
\hline\hline
FEROS  &  $48\,000$ & $350$\, & $920$  & 167\,\, & \,\,45  \\
HARPS  & $115\,000$ & $378$\, & $691$  & 138\,\, & \,\,\, 0 \\
ELODIE &  $45\,000$ & $385$\, & $680$  &  45\,\, & \,\,\, 0 \\
SOPHIE &  $75\,000$ & $387$\, & $694$  &  62\,\, & \,\,62  \\
UVES   & $110\,000$ & $300$\, & $1100$ & 277\,\, & \,\,\, 0 \\
CAFE   &  $62\,000$ & $407$\, & $925$  &  34\,\, & \,\,34  \\
\hline\hline
\end{tabular}
\tablefoot{Number of spectra analysed and number of new spectra obtained in this study with different instruments. The total number of spectra analysed is 723 and 141 of them are new. The (maximum) resolving power and spectral range of each spectrograph are indicated.}
% \tablefoot{Some sources have been observed several times with the same or various instruments. In the case of multiple spectra for the same star we compute the radial velocities as described in Sect.~\ref{section2.3.2}.}
\end{table}
